MFED: A System for Monitoring Family Eating Dynamics

Obesity is a risk factor for many health issues, including heart disease, diabetes, osteoarthritis, and certain cancers. One of the primary behavioral causes, dietary intake, has proven particularly challenging to measure and track. Current behavioral science suggests that family eating dynamics (FED) have high potential to impact child and parent dietary intake, and ultimately the risk of obesity. Monitoring FED requires information about when and where eating events are occurring, the presence or absence of family members during eating events, and some person-level states such as stress, mood, and hunger. To date, there exists no system for real-time monitoring of FED. This paper presents MFED, the first of its kind of system for monitoring FED in the wild in real-time. Smart wearables and Bluetooth beacons are used to monitor and detect eating activities and the location of the users at home. A smartphone is used for the Ecological Momentary Assessment (EMA) of a number of behaviors, states, and situations. While the system itself is novel, we also present a novel and efficient algorithm for detecting eating events from wrist-worn accelerometer data. The algorithm improves eating gesture detection F1-score by 19% with less than 20% computation compared to the state-of-the-art methods. To date, the MFED system has been deployed in 20 homes with a total of 74 participants, and responses from 4750 EMA surveys have been collected. This paper describes the system components, reports on the eating detection results from the deployments, proposes two techniques for improving ground truth collection after the system is deployed, and provides an overview of the FED data, generated from the multi-component system, that can be used to model and more comprehensively understand insights into the monitoring of family eating dynamics.

==> tex_files/4_0_location_detection.tex <==
\section{Location Detection}
To be added

==> tex_files/5_2_4_localization.tex <==
\subsubsection{\textbf{Localization:\\}}
To be added

==> tex_files/9_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
To be added
%M2FED attempts a dramatically different mHealth approach to obesity by not focusing directly on diet and activity, but rather on family eating dynamics (FED). This poster presents the architecture of the monitoring system for FED and some of the major challenges toward implementing such a system.  With the capacity of delivering highly personalized, just-in-time, adaptive interventions, the system would have a downstream positive impact on diet and ultimately obesity.


==> tex_files/acknowledgments.tex <==
\section*{ACKNOWLEDGMENTS}
This work was supported, in part, by NSF Grant CNS-1646470 and DGIST Research and Development Program (CPS Global Center) funded by the Ministry of Science, ICT \& Future Planning.


==> tex_files/copyright_note.tex <==
\copyrightyear{2019}
\setcopyright{acmcopyright}
\acmConference[IMWUT]{PACM Interact. Mob. Wearable Ubiquitous Technol.}{May 2019}{}
\acmISBN{...}
%\acmPrice{\$15.00}
\acmDOI{...}


==> tex_files/draft.tex <==

\begin{figure}\centering
\includegraphics[width=0.9\linewidth]{figures/deployment/daily_plot_1.png}
\caption{Data from the watch and the EMAs for a participant over a day.}
\label{fig:daily_plot_1}
\end{figure}


\begin{figure}\centering
\includegraphics[width=0.9\linewidth]{figures/deployment/daily_plot_2.png}
\caption{An example of a day where the participant used the watch for few hours over a day.}
\label{fig:daily_plot_2}
\end{figure}

\begin{table}
\begin{tabular}{|c|c|}
\hline
\textbf{With} & \textbf{Count} \\ \hline
Nobody & 97\\ \hline
Spouse/Partner, Child(ren) & 48 \\ \hline
Child(ren) & 22 \\ \hline
Mother, father, brother(s) & 16 \\ \hline
Brother(s) & 15 \\ \hline
Spouse/partner & 14 \\ \hline
mother & 10\\ \hline

\end{tabular}
\caption{Instance counts for Group of People eating with the participant responded to the eating EMA}
\label{table:with_whom}
\end{table}


\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/deployment/mindful_eating/mindful_tod_bar_1.png}
  \caption{}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/deployment/mindful_eating/mindful_dow_bar_1.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\caption{Responses to "My thoughts were wandering while I ate"  for different (a) time of the day and (b) days of the week}
\label{fig:mindful_1}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/deployment/mindful_eating/mindful_tod_bar_2.png}
  \caption{}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/deployment/mindful_eating/mindful_dow_bar_1.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\caption{Responses to "I was thinking about things I need to do while I ate"  for different (a) time of the day and (b) days of the week}
\label{fig:mindful_2}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/deployment/mindful_eating/mindful_tod_bar_2.png}
  \caption{}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/deployment/mindful_eating/mindful_dow_bar_1.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\caption{Responses to "I ate so quickly that I didn't taste anything"  for different (a) time of the day and (b) days of the week}
\label{fig:mindful_3}
\end{figure}


*** Please share your thoughts on what kind of insights or analysis we should put here.


%===============================
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{} & \textbf{Upset} & \textbf{Nervous} & \textbf{Stressed} & \textbf{Couldn't cope} \\ \hline 
Happy & -0.23 & -0.14 & -0.16 & -0.15\\ \hline
Great & -0.24 & -0.15 & -0.25 & -0.16 \\ \hline
Cheerful & -0.26 & -0.16 & -0.27 & -0.16 \\ \hline
Joyful & -0.24 & -0.15 & -0.27 & -0.15 \\ \hline
\end{tabular}
\caption{Correlation coefficients between the responses to the queries for positive affect states and perceived stress.}
\label{table:affect_vs_states}
\end{table}

==> tex_files/x_5_2_4_mindful_eating.tex <==
\subsubsection{Mindful Eating:}
There are three EMA queries related to mindful eating that are asked when an eating event is detected correctly. Table \ref{table:mindful_eating} shows the questions  and responses to the questions. The numbers in the parentheses represent the counts when the participants ate alone. During most of the eating events, the participants' thoughts did not wonder and they did not think about other things that they needed to do. Also, there are very few eating events where the participants ate quickly. This result shows that people eat mindfully most of times, particularly at home. Eating together has significant impact on mindful eating. We see that the participants thought about things to do or their thoughts were wondering more while eating alone than eating with others. Though there are very few eating events when the participants ate quickly, they were alone for almost all these events. These examples illustrate the influence of family eating dynamics on eating behavior.    

\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Query} & \textbf{Very} & \textbf{Somewhat} & \textbf{A Little} & \textbf{Not} \\ 
\textbf{} & \textbf{True} & \textbf{True} & \textbf{True} & \textbf{True} \\ \hline
My thoughts were wandering while I ate & 33 (24) & 33 (18) & 81 (44) & 154 (68) \\ \hline
I was thinking about things I need to do while I ate & 28 (20) & 38 (23) & 90 (49) & 145 (62) \\ \hline
 I ate so quickly that I didn't taste anything & 5 (5) & 6 (5) & 19 (8) & 271 (136)\\ \hline
\end{tabular}
\caption{The response counts for mindful eating. The numbers in the parentheses represent the counts when the participants ate alone.}
\label{table:mindful_eating}
\end{table}




==> tex_files/x_5_2_5_perceived_stress.tex <==
\subsubsection{Perceived Stress:}
The participants were asked about their perceived stress states (upset, nervous, stressed, and couldn't cope) both for the mood and the eating EMAs. The summary of the responses for this query is given in Table \ref{table:stress_scale}. The number of EMA responses with higher perceived stress states is much less compared to little or no perceived states. Among the perceived states, feeling stressed is more prevalent than others. The counts of perceived states with rating `very' and `some' for the individuals are shown in Figure \ref{fig:perceived_stress_all}. We see that most of the perceived stress states with a higher rating (`very' and `some') come from only a few of the participants. In order to better understand the correlation between mindful eating and perceived stress, the correlation coefficient between the responses to the queries are listed in Table \ref{table:mindful_vs_stress}. Results show that lack of mindfulness (thoughts wandering, thinking about things to do, or eating quickly) are weakly correlated with perceived stress.  

\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Perceived Stress} & \textbf{Very} & \textbf{Some} & \textbf{A little} & \textbf{Not at all} \\ \hline
Upset & 45 & 116 & 400 & 3208 \\ \hline
Nervous & 15 & 100 & 390 & 3272 \\ \hline
Stressed & 64 & 262 & 673 & 2779 \\ \hline
Couldn't cope & 14 & 87 & 247 & 3431 \\ \hline
\end{tabular}
\caption{The response counts for different degree of the perceived stress.}
\label{table:stress_scale}
\end{table}


%==========================
\begin{figure}\centering
\includegraphics[width=0.9\linewidth]{figures/deployment/perceived_stress/all_very_some.png}
\caption{The response count for the perceived stress (very and some) of individuals.}
\label{fig:perceived_stress_all}
\end{figure}


%==========================

\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Query} & \textbf{Upset} & \textbf{Nervous} & \textbf{Stressed} & \textbf{Couldn't cope} \\ \hline 
My thoughts were wandering while I ate & 0.14 & 0.21 & 0.22 & 0.15 \\ \hline
I was thinking about things I need to do while I ate & 0.18 & 0.23 & 0.21 & 0.23 \\ \hline
 I ate so quickly that I didn't taste anything & 0.14 & 0.11 & -0.05 & 0.12\\ \hline
\end{tabular}
\caption{The correlation coefficients between the responses to mindful eating and perceived stress.}
\label{table:mindful_vs_stress}
\end{table}

==> tex_files/x_5_2_6_positive_affect.tex <==
\subsubsection{Positive Affect States:}
The participants were asked about positive affect states (happy, great, cheerful, and joyful) in the hourly mood EMA surveys. The summary of the responses is shown in Table \ref{table:stress_scale}. In contrast to the perceived stress states that are reported mostly as 'a little' or 'Not at all', the positive affect states are more evenly distributed among different degrees (very, some, a little and not at all). To get insight into the affect states for the families and the individuals, the response ratios for different degrees of Happiness for the individuals are plotted in Figure \ref{fig:happiness_degree}. We get similar results for other affect states(great, cheerful, and joyful), and do not show them here to avoid redundancy. From the figure, we see that positive affect states of family members are highly correlated for most of the families. It indicates the influence of family members on each other regarding affect states.

%The correlation coefficient between the responses to the queries for positive affect states and perceived stress are listed in Table \ref{table:afect_vs_stress}. As expected, these two group of states are negatively correlated.

\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Affect} & \textbf{Very} & \textbf{Some} & \textbf{A little} & \textbf{Not at all} \\ \hline
Happy & 1017 & 1164 & 728 & 562\\ \hline
Great & 1023 & 985 & 704 & 762 \\ \hline
Cheerful & 939 & 976 & 648 & 911 \\ \hline
Joyful & 943 & 919 & 675 & 937 \\ \hline
\end{tabular}
\caption{Count of EMA responses for different degrees of positive affect state.}
\label{table:positive_affect}
\end{table}



%==========================
\begin{figure}\centering
\includegraphics[width=0.9\linewidth]{figures/deployment/affect/happy_ratio_individual.png}
\caption{The ratios of the degrees of happiness for the individuals}
\label{fig:happiness_degree}
\end{figure}



==> tex_files/x_5_2_7_EAH.tex <==
\subsubsection{Eating in the Absence of Hunger:}
Eating in the absence of hunger (EAH) is a major factor for weight gain \cite{kral2010adolescent}. It refers to the phenomenon of eating foods when satiated. The eating EMA survey asks the participants for the reasons behind EAH. The list of reasons asked and the summary of the responses from the participants are given in Table \ref{table:eah}. We see that physical or mental states like feeling bored, tired, sad, and anxious sometimes result in EAH. But, the most dominant reason is that the food looked, tasted or smelled so good. People's desire to finish the food on the plate or to eat with others are also among the major reasons for EAH. Family or parents also influence EAH significantly. The dominant reasons of EAH for different families or individuals are different. The responses to the EMA queries related to EAH give insight into the reasons that should be targeted to reduce EAH effectively for a family or for an individual.  

\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Serial} & \textbf{Reason} & \textbf{Very True} & \textbf{Somewhat true} & \textbf{A little true} & \textbf{Not true}\\ \hline
1 & Food looked, tasted or smelled so good & 75 & 70 & 60 & 96\\ \hline
2 & Others were eating & 30 & 33 & 38 & 200 \\ \hline
3 & Feeling sad or depressed & 4 & 2 & 14 & 280\\ \hline
4 & Feeling bored  & 8 & 13 & 35 & 245 \\ \hline
5 & Feeling angry or frustrated & 4 & 2 & 14 & 280 \\ \hline
6 & Feeling tired & 12 & 17 & 42 & 230 \\ \hline
7 & Feeling anxious or nervous & 5 & 4 & 16 & 276\\ \hline
8 & My family or parents wanted me to eat & 16 & 32 & 17 & 236 \\ \hline
9 & I wanted to finish the food on my plate & 47 & 52 & 43 & 159\\ \hline
\end{tabular}
\caption{Reasons for eating in the absence of hunger and summary of the responses}
\label{table:eah}
\end{table}


==> tex_files/x_5_2_8_hunger_full.tex <==
\subsubsection{Hunger and Fullness:}
The participants were asked how hungry they are before, and full after eating. A slider (with 0-100 scale where 0 is not at all and 100 is completely) is available in the EMA app for input. Figures \ref{fig:hunger_state} (a) and \ref{fig:hunger_state} (b) show the histogram of hunger and fullness, respectively, where the y axis represents the count of eating events for the bins. The mean values of hunger and fullness are 51 and 60 with standard deviation 22 and 23, respectively. The data shows that hunger and fullness differ significantly for the eating events. Interestingly, people often eat when they are not very hungry and are often not completely full when finishing. 

\begin{figure}[H]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/deployment/hunger/hunger_before_eat.png}
  \caption{}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/deployment/hunger/full_after_eat.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\caption{Histograms of eating events with (a) Hunger before, and (b) full after eating}
\label{fig:hunger_state}
\end{figure}



